Quantitative Stability of Optimal Transport Maps under Variations of the Target Measure

This work studies the quantitative stability of the quadratic optimal transport map between a fixed probability density $\rho$ and a probability measure $\mu$ on R^d , which we denote T$\mu$. Assuming that the source density $\rho$ is bounded from above and below on a compact convex set, we prove that the map $\mu$ $\rightarrow$ T$\mu$ is bi-H{\"o}lder continuous on large families of probability measures, such as the set of probability measures whose moment of order p > d is bounded by some constant. These stability estimates show that the linearized optimal transport metric W2,$\rho$($\mu$, $\nu$) = T$\mu$ -- T$\nu$ L 2 ($\rho$,R d) is bi-H{\"o}lder equivalent to the 2-Wasserstein distance on such sets, justifiying its use in applications.

==> 6_kmeans.tex <==
\label{sec:kmeans}
We give in this section an illustrative application of the proven bi-Hölder stability result to a classical data analysis task of clustering in the space of probability measures endowed with the Wasserstein distance. Several applications involve decomposing a finite family of probability measures into clusters, using the $p$-Wasserstein distances as a guiding geometry. These applications include classification of images \cite{wass-kmeans-simplex, wass-kmeans-fast, wass-kmeans-multilevel}, of tomographic projections  \cite{wass-kmeans-tomographic}, of time-series \cite{wass-kmeans-inter-arrival, wass-kmeans-multilevel}, of textual documents \cite{wass-kmeans-fast} or of cloud regime histograms \cite{wass-kmeans-cloud}. In order to keep the computational cost reasonable, many of these works involve approximations that are not analyzed theoretically in terms of clustering quality. The objective of this section is to establish a (simple) guarantee on the clustering quality that one can obtain in the Linearized Optimal Transport framework, relying on  Theorem~\ref{th:stability-ot-maps}.

\subsection*{\texorpdfstring{$K$}{}-means clustering in metric spaces}
In a general metric space $(M, d_M)$, the $K$-Means clustering of $N$ data points $x_1, \dots, x_N \in M$ consists in finding a set of $K$ centroids (also called \emph{means}) $\bm{c} = (c_1, \dots, c_K) \in M^K$ minimizing the \emph{distortion}
$$ R_M(\bm{c}) = \frac{1}{N} \sum_{i=1}^N \min_{j=1, \dots, K} d_M(x_i, c_j)^2.$$
A set of centroids $\bm{c} \in M^K$ induces a clustering of the set $\{x_i\}_{1\leq i\leq N}$ using Voronoi cells:
$$\forall j \in \{1, \dots, K\}, \quad V_j(\bm{c}) = \{ x_i \mid \forall \ell \in\{1,\hdots,K\}, d_M(x_i, c_j) \leq d_M(x_i, c_\ell) \}.$$
%allowing to rewrite the $K$-Means energy as 
%$$ R_M(\bm{c}) = \frac{1}{N} \sum_{j=1}^K \sum_{x_i \in V_j(\bm{c})} d_M(x_i, c_j)^2.$$
The $K$-Means clustering problem thus consists in finding a clustering of the data at hand that minimizes the within-cluster variance, obtained by minimizing $R_M$.
A popular algorithm used to find a local minimum of $R_M$ is Lloyd's algorithm \cite{Lloyd}. However, because of its non-convexity, minimizing the objective $R_M$ is in general NP-hard \cite{kmeans-np-hard}. Performance guarantees in terms of clustering error for $K$-means algorithms can still be obtained, but only  under assumptions of well-clusterabilty of the data and good initialization of the centroids.
A popular initialization method is offered by the $K$-Means$++$  \cite{kmeans++} randomized seeding technique, and is described in Algorithm \ref{alg:kmeans++}.

%commonly known as the $K$-means clustering algorithm, which from a set of initial centroids alternates between the computation of the Voronoï cell of each centroid and the update of each centroid with the barycenter of its associated Voronoï cell.
%These updates are known to decrease the $K$-means objective $R_M$ and Lloyd's algorithm can thus be viewed as a local descent algorithm. However the objective $R_M$ is in general NP-hard to optimize \cite{kmeans-np-hard} and performance guarantees in term of clustering error for $K$-means algorithms can only be obtained under assumptions of well-clusterabilty of the data and good initialization of the centroids.

%This technique consists in choosing a first centroid $c_1$ uniformly at random from $\{x_1, \dots, x_N\}$, and then, from $j=2$ to $j=K$, selecting $c_j = x_i \in \{x_1, \dots, x_N\}$ with probability $d_M(x_i, \bm{c}_{1:j-1})^2 / \sum_{i'=1}^N d_M(x_{i'}, \bm{c}_{1:j-1})^2$, where $\bm{c}_{1:j-1} = \{c_1, \dots, c_{j-1}\}$.

\begin{algorithm}
\SetAlgoLined
%\KwData{Dataset $\{x_1, \dots, x_N\}$}
%\KwResult{Set of initialized centroids $\bm{\hat{c}}$}
 Select an initial centroid $\hat{c}_1$ uniformly at random from $\{x_1, \dots, x_N\}$ and set $\mathcal{C}_1 = \{\hat{c}_1\}$\;
 \For{$j \leftarrow 2$ \KwTo $K$}{
 Select $\hat{c}_j = x_i \in \{x_1, \dots, x_N\}$ with probability $\frac{d_M(x_i, \mathcal{C}_{j-1})^2}{\sum_{i'=1}^N d_M(x_{i'}, \mathcal{C}_{j-1})^2}$\;
 Set $\mathcal{C}_{j} = \mathcal{C}_{j-1} \cup \{\hat{c}_j\}$\;
 }
 \caption{$K$-Means$++$ randomized seeding technique \cite{kmeans++}}
 \label{alg:kmeans++}
\end{algorithm}



The (random) output $\bm{\hat{c}} = (\hat{c}_1, \dots, \hat{c}_K)$ of Algorithm~\ref{alg:kmeans++} comes with the following guarantee in expectation in term of the $K$-Means objective (\cite{Nielsen2019}, Theorem 4): 
\begin{equation} \label{eq:kmeansppguarantee}
    \Esp_{\bm{\hat{c}}} R_M(\bm{\hat{c}}) \leq 16(\log K + 2) \min_{\bm{c} \in M} R_M(\bm{c}).
\end{equation} where $\Esp_{\bm{\hat{c}}}$ denotes the expectation w.r.t. the random variable $\bm{\hat{c}}$ following the law described in Algorithm~\ref{alg:kmeans++}. Combined with clusterability assumptions, this estimate yields performance guarantees in terms of clustering quality when using $\bm{\hat{c}}$ as a set of centroids.
\begin{theorem}
\label{th:kmeans++}
Let $x_1, \dots, x_N \in M$ partitioned into $K'$ disjoint non-empty clusters $(C_j)_{j=1, \dots, K'}$, and assume that there exists $\epsilon > 0$ and $f \geq 1$ such that for all $\ell, \ell' \in \{1, \dots, K'\}$ with $\ell \neq \ell'$,
\begin{align*}
    \forall (x_i, x_j) \in C_\ell \times C_\ell, \quad d_M(x_i, x_j) &\leq \epsilon,\\
    \forall (x_i, x_j) \in C_\ell \times C_{\ell'}, \quad d_M(x_i, x_j) &\geq f \epsilon.
\end{align*}
Denote $\bm{\hat{c}}$ the set of centroids given by the $K$-Means$++$ seeding and $\tau_{err}(\bm{\hat{c}})$ the proportion of misclassified points using the centroids $\bm{\hat{c}}$, i.e.
$$\tau_{err}(\bm{\hat{c}}) = \frac{1}{N} \sum_{j=1}^K \min_{j' = 1, \dots, K'} \abs{ V_{j}(\bm{\hat{c}}) \cap \left(C_{j'}\right)^C}.$$
Then for $g \geq 1$, we have %, with probability greater than $1 - \frac{16(\log K + 2)g}{f^2}$,
$$ \Proba_{\bm{\hat{c}}}\left(\tau_{err}(\bm{\hat{c}}) \leq \frac{1}{g}\right) \geq 1 - \frac{16(\log K + 2)g}{f^2}$$
\end{theorem}
%\textcolor{red}{$\mathfrak{S}(K)$}
\begin{proof}
First notice that Markov's inequality and the $K$-Means$++$ guarantee \eqref{eq:kmeansppguarantee} ensure $$\Proba_{\bm{\hat{c}}}\left(R_M(\bm{\hat{c}}) \geq \frac{f^2}{g} \min_{\bm{c} \in M} R_M(\bm{c}) \right) \leq \frac{g \Esp_{\bm{\hat{c}}} R_M(\bm{\hat{c}})}{f^2 \min_{\bm{c} \in M} R_M(\bm{c})} \leq \frac{16(\log K + 2) g}{f^2}.$$
Thus with probability greater than $1 - \frac{16(\log K + 2)g}{f^2}$, we have $R_M(\bm{\hat{c}}) \leq \frac{f^2}{g} \min_{\bm{c} \in M} R_M(\bm{c}).$
However, the clusterability assumptions imply that
\begin{equation*}
    \min_{\bm{c} \in M} R_M(\bm{c}) \leq \epsilon^2 \quad \text{and} \quad R_M(\bm{\hat{c}}) \geq \tau_{err}(\bm{\hat{c}}) f^2 \epsilon^2.
\end{equation*}
%$$ \min_{\bm{c} \in M} R_M(\bm{c}) \leq \epsilon^2,$$
%$$ R_M(\bm{\hat{c}}) \geq \tau_{err}(\bm{\hat{c}}) f^2 \epsilon^2. $$
Hence with probability greater than $1 - \frac{16(\log K + 2)g}{f^2}$, $\tau_{err}(\bm{\hat{c}}) f^2 \epsilon^2 \leq \frac{f^2}{g} \epsilon^2.$
%\begin{equation*}
%    \tau_{err}(\bm{\hat{c}}) f^2 \epsilon^2 \leq \frac{f^2}{g} \epsilon^2. \qedhere 
%\end{equation*}
\end{proof}
%\begin{remark}
%This result gives very strong guarantees for $f^2 \gg \log K$.
%\end{remark}

\subsection*{\texorpdfstring{$K$}{}-Means with Linearized OT} The performance guarantee given in Theorem \ref{th:kmeans++} holds for a general metric space $(M, d_M)$ and it is thus possible to choose $(M, d_M) = (\Prob_2(\Rsp^d), \Wass_2)$. A dataset $\mu_1, \dots, \mu_N \in (\Prob_2(\Rsp^d), \Wass_2)$ satisfying the clusterability assumptions of Theorem \ref{th:kmeans++} can therefore be clustered with the $K$-Means$++$ seeding at the cost of solving $O(KN)$ optimal transport problems in order to compute the seeding probabilities. For settings with relatively large values of \textcolor{blue}{$N$ or} $K$, these computations might be prohibitive and it might be interesting to choose to embed $(\Prob_2(\Rsp^d), \Wass_2)$ into $\L^2(\rho; \Rsp^d)$ using the mapping $\mu \mapsto T_\mu$. Indeed, doing this requires solving only $N$ optimal transport problems to compute the embeddings and then computing $O(KN)$ Hilbertian distances. Moreover, optimal transport problems between a probability density over a convex set and a point cloud can be solved in dimension $d=2,3$ very efficiently, with a cost that is empirically linear in the cardinal of the point cloud \cite{kitagawa:hal-01290496}. Performance guarantees for $K$-Means$++$ seeding on the dataset $T_{\mu_1}, \dots, T_{\mu_N} \in \L^2(\rho; \Rsp^d)$  can still be obtained from Theorem \ref{th:kmeans++} by assuming stronger clusterability assumptions on the dataset $\mu_1, \dots, \mu_N \in (\Prob_2(\Rsp^d), \Wass_2)$. Indeed, assume first that $\mu_1, \dots, \mu_N$ belong to a subset $S \subset \Prob_2(\Rsp^d)$ that is such that there exists $(C_S, \alpha_S) \in \Rsp^*_+ \times (0, 1)$ such that $$ \forall \mu, \nu \in S, \quad \Wass_2(\mu, \nu) \leq \nr{T_\mu - T_\nu}_{\L^2(\rho)} \leq C_S \Wass_2(\mu, \nu)^{\alpha_S}.$$ Theorem \ref{th:stability-ot-maps} and Corollary \ref{cor:embedding-BWp-Mp} give examples of such sets $S$. Then assume that $\mu_1, \dots, \mu_N$ is partitioned into $K$ disjoint non-empty clusters $(C_j)_{j=1, \dots, K}$, and that there exists $\epsilon > 0$ and $f \geq 1$ such that for all $\ell, \ell' \in \{1, \dots, K\}$ with $\ell \neq \ell'$,
\begin{align*}
    \forall (\mu_i, \mu_j) \in C_\ell \times C_\ell, \quad \Wass_2(\mu_i, \mu_j) &\leq \left( \frac{\epsilon}{C_S}\right)^{1/\alpha_S},\\
    \forall (\mu_i, \mu_j) \in C_\ell \times C_{\ell'}, \quad \Wass_2(\mu_i, \mu_j) &\geq f \epsilon.
\end{align*}
Then one can apply Theorem \ref{th:kmeans++} to the dataset $T_{\mu_1}, \dots, T_{\mu_N} \in \L^2(\rho; \Rsp^d)$.

\begin{figure}
    \centering
    \includegraphics[width=.6\textwidth]{figures/examples_emnist.pdf}  \\
    \includegraphics[width=.6\textwidth]{figures/centroids_emnist.pdf} 
    \caption{(Top) Example images of upercase A, B, and C from the EMNIST \cite{emnist} dataset. (Bottom) Push-forwards of the $6$ centroids.}
    \label{fig:kmeans}
\end{figure}

We finally give an illustration of the described techniques by performing a clustering of images of handwritten letters. We extract from the EMNIST \cite{emnist} dataset $2,000$ images of each of the uppercase letters A, B and C (Figure \ref{fig:kmeans}) and convert each image into a discrete probability measure of $\X = [0, 1]^2$ by treating the pixels as Dirac masses. Taking $\rho$ to be the Lebesgue measure on $\X$, we then compute for each measure its optimal transport map from $\rho$ to itself. We eventually perform a clustering with the $K$-means$++$ algorithm on the
vectorized maps, looking for $K = 6$ clusters. The push-forwards of the $6$ centroids are shown in Figure \ref{fig:kmeans} where each \textit{class} seems to be recovered and where \textit{intra-class}
variation might be explained from the use or not of italic writing.




%We note that embedding $(\Prob_2(\Rsp^d), \Wass_2)$ into $\L^2(\rho; \Rsp^d)$ is also computationally advantageous for continuing the $K$-Means algorithm with Lloyd's update after initializing with $\bm{c^{++}}$, alternating between the computation of $KN$ distances and the computation of $K$ barycenters. Other performance guarantees are available when doing so, see \cite{kmeans-guarantee, levrard:hal-01667014}.\\
%We conclude this section with an illustration of the algorithm ....

% Énergie minimale: E_0 <= eps^2
% Énergie garantie par k-means++: E_{k++} <~ (ln k + 2) eps^2
% S'il manque un centroide dans un cluster => erreur = pourcentage de données dans le cluster * D^2 (D = distance inter-cluster)
% S'il manque un point dans une proportion >= alpha des clustes => énergie >= alpha D^2
% Impossible si alpha D^2 > 8(ln k + 2) eps^2
% alpha  <= 8(ln k+2)/f^2

%\textcolor{red}{
%Garantie existe déjà dans \cite{wass-kmeans-cloud}. Provient de \cite{Nielsen2019}, qui donne résultat sur kmeans++ dans un espace métrique quelconque (Théorèmes 3 et 4 de la version arxiv)\\ \\
%Consider $\mu_1, \dots, \mu_N \in (\Prob_2(\Rsp^d), \Wass_2)$ such that for $f \geq 1$
%$$\forall (i,j) \in C_\ell \times C_\ell, \nr{T_{\mu_i} - T_{\mu_j}}_{\L^2(\rho)} \leq \eps,$$
%$$ \forall (i,j) \in C_\ell \times C_{\ell'}, \nr{T_{\mu_i} - T_{\mu_j}}_{\L^2(\rho)} \geq f \eps.$$
%Then $\min_{c} R_{\L^2(\rho)}(c) \leq \eps^2$. And any set of centroids that has a point in each cluster of the dataset gives the optimal clustering ($C_\ell = V_\ell$). Thus if $K$-Means$++$ gives a clustering with a proportion $\tau \in (0, 1]$ of misclassified points, the associated cost is at least $R_{\L^2(\rho)}(c^{++}) \geq \tau f^2 \eps^2$. However we have (Theorem 3.1 \cite{wass-kmeans-cloud}) for $c^{++}$ the set of centroids given by the $K$-Means$++$ algorithm:
%$$ \Esp_{c^{++}} R_{\L^2(\rho)}(c^{++}) \leq 8(\log K + 2) \min_{c} R_{\L^2(\rho)}(c)\leq 8(\log K + 2)\eps^2. $$
%Thus we have, using Markov's inequality:
%\begin{align*}
%    \Proba_{c^{++}}(\text{"$\tau\%$ of misclassification"}) &\leq \Proba_{c^{++}}(R_{\L^2(\rho)}(c^{++}) \geq \tau f^2 \eps^2)\\
%    &\leq \frac{8(\log K + 2)}{\tau f^2}
%\end{align*}
%}
